Accelerating Transfer Learning with Near-Data Computation on Cloud Object Stores

Storage disaggregation underlies today's cloud and is naturally complemented by pushing down some computation to storage, thus mitigating the potential network bottleneck between the storage and compute tiers. We show how ML training benefits from storage pushdowns by focusing on transfer learning (TL), the widespread technique that democratizes ML by reusing existing knowledge on related tasks. We propose HAPI, a new TL processing system centered around two complementary techniques that address challenges introduced by disaggregation. First, applications must carefully balance execution across tiers for performance. HAPI judiciously splits the TL computation during the feature extraction phase yielding pushdowns that not only improve network time but also improve total TL training time by overlapping the execution of consecutive training iterations across tiers. Second, operators want resource efficiency from the storage-side computational resources. HAPI employs storage-side batch size adaptation allowing increased storage-side pushdown concurrency without affecting training accuracy. HAPI yields up to 2.5x training speed-up while choosing in 86.8% of cases the best performing split point or one that is at most 5% off from the best.

==> scratchpad.tex <==
\section{Related Work}
\label{sec:related-work}

\system{} contains a unique combination of context (\objstore{}), workload (TL), and design decisions (splitting a DNN between cloud tiers, batch adaptation). While related work exists in these directions, \system{} is the first to combine them in a single cohesive system.
%{\color{red} why works of other applications/domain could not be applied directly to our case?}

\vspace{0.07in}\noindent{\bf Batch adaptation in ML. }


Several projects~\cite{mascots20-ibm, iclr2018-GoogleIncreaseBatch,kdd2017-batch} proposed to dynamically adapt the \emph{training} batch size as training proceeds, leading to shorter training times without loss in accuracy. These ideas are complementary to \system{}'s batch adaptation because they can be applied in \system{}'s training phase. Instead, the key insight of batch adaptation in \system{} is that during the same iteration, it is useful to use different batch sizes for feature extraction compared to training.

\vspace{0.07in}\noindent{\bf Splitting compute between edge and cloud. }
Neurosurgeon~\cite{kang2017neurosurgeon} splits ML \emph{inference} between the cloud and edge devices to achieve low latency, low energy consumption, and high data center throughput. The partitioning is automatic and adapts to dynamics in server load and network bandwidth. Compared to Neurosurgeon, besides considering more complex application (i.e., TL), \system{} dynamically manages storage-side concurrency via batch adaptation. MAUI~\cite{mobisys10-maui} performs fine-grained (function-level) energy-aware offload of mobile code to the infrastructure, via runtime decisions driven by the goal to save energy. MAUI's approach to splitting cannot be directly used in \system{} because it requires programmer annotations, and transfers all program state including variables. Odessa~\cite{mobisys11-odessa} offloads stages in perception applications but without analyzing the global impact on application~performance.

\vspace{0.07in}\noindent{\bf Offloading compute to storage nodes. }
Rhea~\cite{nsdi2013-rhea} uses static analysis of Java bytecode to generate storage-side filters for Hadoop applications. Rhea shares the goal of mitigating the network bottleneck to storage but targets a different workload, does not split an application and does not optimize the resource utilization in the storage layer. Pyxis~\cite{vldb2012-madden-partitioning} uses static analysis and dynamic runtime information to automatically partition a database application between application and storage nodes. Pyxis automatically generates database-side stored procedures to minimize overall latency subject to CPU constraints. For this, it minimizes the number of control transfers as well as amount of data sent during each control transfer. Pyxis differs in the application, context, and concerns (i.e., control transfers are specific to database applications).





%Rhea~\cite{nsdi2013-rhea} automatically generates and runs storage-side data filters for unstructured and semi-structured data. Given a Hadoop-like application, Rhea uses static analysis of Java bytecode to generate stateless storage-side filters that remove, in a best-effort fashion, useless data for the computation. While the goal to relieve the cloud storage bottleneck is similar to ours, Rhea focuses on a different class of applications, does not actually split an application, and does not optimize the resource utilization in the storage layer.

%Pyxis~\cite{vldb2012-madden-partitioning} uses static analysis and dynamic runtime information to automatically partition a database application between application and storage nodes. Pyxis automatically generates database-side stored procedures with the goal of minimizing overall latency subject to CPU resource constraints. Key to Pyxis is minimizing the number of control transfers as well as amount of data sent during each control transfer. Pyxis differs from \system{} in the application, context and concerns (i.e. control transfers are specific to database applications). 

%Hadoop2SQL~\cite{eursys10-willy-HadoopToSql} aims to improve MapReduce performance, in particular the workloads that selectively access data, by transforming the entire MapReduce program, or parts of it, into an SQL query that can leverage the efficient operator implementations inside SQL databases. Hadoop2SQL is only similar to \system{} at the very high level; the setting and the applications are different. Hadoo2SQL has a strong focus on static analysis and does not optimize storage-side metrics.

\vspace{0.07in}\noindent{\bf Computation pushdown in \objstore{}. }
Work on pushing down computation in the \objstore{} mainly focuses on how to best leverage the limited subset of SQL supported by Amazon S3 Select-like systems since 2017. PushdownDB~\cite{icde2020-pushdowndb} analyzes which DBMS primitives can be cost-effectively moved into S3 and how more complex operations (e.g., joins) can be re-implemented to take advantage of S3 Select. FlexPushdownDB~\cite{vldb2021-flexpushdowndb} combines the benefits of caching and computation pushdown for query execution (e.g., Star Schema Benchmark) by introducing a separable operator and a new cache replacement policy that takes into account the cost of pushdowns.



\vspace{0.07in}\noindent{\bf Systems challenges for TL. }
Cartel~\cite{socc2019-cartel} provides collaborative TL at the edge by transferring knowledge across geographically distributed edge clouds while minimizing transfers over the backhaul network. Cartel differs as it focuses on challenges in learning at the edge, e.g., detecting similarities between edge clouds and performing the knowledge transfer. NDPipe~\cite{ndpipe-asplos24} is a parallel effort to ours focusing on accelerating training and inference for image data by using near-data processing techniques to photo storage servers equipped with inexpensive commodity GPUs. \system{} differs in several technical aspects, notably by analyzing concurrency in the \objstore{}, proposing storage-side batch size adaptation, avoiding OOMs and by fine-tuning without impacting the accuracy.

%references about how to solve memory problems -- we do batch adaptation for that
%\item \url{https://www.usenix.org/conference/fast21/presentation/bae} -- interesting -- uses SSD in DNN training -- another way to solve the memory problems (they say one solution is to use host memory -- for offloading) yet, this paper uses fast SSD to solve the GPU memory problem. It depends on a direct very fast links between SSD and GPU though. This can be used as a reference to the GPU memory problem (see Fig. 2 in the paper).
%there should be also other papers that use the host memory and pipelining to solve this problem -- we can check that later.

\vspace{0.07in}\noindent{\bf Model/pipeline parallelism.}
Splitting in \system{} is reminiscent of model and pipeline parallelism, which aim to distributedly train large models. Model parallelism ~\cite{projectadam-osdi14} splits a DNN across workers. This is a form of intra-batch parallelism as all workers process the same batch. Pipeline parallelism~\cite{pipedream-sosp19,gpipe-neurips19} further improves the efficiency of model parallelism. Pipedream~\cite{pipedream-sosp19} combines intra with inter-batch parallelism (multiple batches execute concurrently) and mitigates staleness and consistency issues by keeping several versions of the weights. GPipe~\cite{gpipe-neurips19} does not do inter-batch parallelism, but splits a single batch into micro-batches and pipelines those.

\system{} differs in several ways. The high-level goal differs as \system{} aims to mitigate the \objstore{} network bottleneck. The approach to splitting differs as the splitting point in \system{} is dynamic but fixed in model/pipeline parallelism. The concerns differ as \system{}'s server handles multiple clients concurrently. The challenges differ as there is no backpropagation on \system{}'s server or between \system{}'s client and server. 

\vspace{0.07in}\noindent{\bf Data ingestion pipelines.}
The feature extraction phase in \system{} is reminiscent of data ingestion/preparation pipelines~\cite{tf.data-vldb2021, data-ingestion-pipelines-isca22-meta-kozyrakis, preprocessing-pipelines-sigmod22} because of their goal (data preparation) and the critical focus on efficiently delivering data for training. However, these pipelines are far more general in nature (e.g., can even run user-defined functions~\cite{tf.data-vldb2021}) and can be very large (e.g., serve data at TB/s~\cite{data-ingestion-pipelines-isca22-meta-kozyrakis}), which makes them unsuitable for running inside the \objstore{}. In \system{}, the main difference is that the feature extraction phase is part of the DNN which, while limiting the knobs available, allows us to focus on accelerating each separate application.






\vspace{1mm}
\begin{algorithm}
    \caption{Choose the split index - runs on client}
    \vspace{3mm}
    \label{alg:choose-split}
    \begin{lstlisting}
If Right before 1st iteration of epoch 0 Then
    split_idx = freeze_idx
    collect profiling data from server & client
    If job failed with OOM Then
        return error to client
    EndIf
EndIf


If Right before mid iteration of epoch 0 Then
    split_idx = earliest split not predicted to cause OOM on client
    collect profiling data from server & client
EndIf


If At end of epoch 0 Then
    runtimes = {}
    For potential_split in [0, freeze_idx]
        If potential_split predicted to NOT cause OOM on client Then
            derive RT_SRV at potential_split from profiling and modeling
            derive RT_CLI at potential_split from profiling and modeling
            derive RT_NW at potential_split from profiling and modeling
            NR_IT = nr iterations in an epoch
            runtimes[potential_split] = RT_SRV + max(RT_SRV + RT_NW, RT_CLI) * (NR_IT - 1) + RT_CLI
        EndIf
    EndFor
    split_idx = idx such that runtimes[idx] is minimized
EndIf
    \end{lstlisting}
    \vspace{1mm}
\end{algorithm}
